Learning Energy-Based Approximate Inference Networks for Structured Applications in NLP

Structured prediction in natural language processing (NLP) has a long history. The complex models of structured application come at the difficulty of learning and inference. These difficulties lead researchers to focus more on models with simple structure components (e.g., local classifier). Deep representation learning has become increasingly popular in recent years. The structure components of their method, on the other hand, are usually relatively simple. We concentrate on complex structured models in this dissertation. We provide a learning framework for complicated structured models as well as an inference method with a better speed/accuracy/search error trade-off. The dissertation begins with a general introduction to energy-based models. In NLP and other applications, an energy function is comparable to the concept of a scoring function. In this dissertation, we discuss the concept of the energy function and structured models with different energy functions. Then, we propose a method in which we train a neural network to do argmax inference under a structured energy function, referring to the trained networks as "inference networks" or "energy-based inference networks". We then develop ways of jointly learning energy functions and inference networks using an adversarial learning framework. Despite the inference and learning difficulties of energy-based models, we present approaches in this thesis that enable energy-based models more easily to be applied in structured NLP applications.

==> Acknowledgements.tex <==
Acknowledgements

==> Background.tex <==
\mychapter{3}{BACKGROUND}
\label{sec:background}

\section{What are Energy-Base Models?}
We denote the space of inputs by $\Xspace$. For a given input $\x\in\Xspace$, we denote the space of legal structured outputs by $\yspace(\x)$. We denote the entire space of structured outputs by $\yspace = \cup_{\x\in\xspace} \yspace(\x)$. 
%an output by $\y\in\yspace(\x)$. 
An \textbf{energy function}~\citep{lecun-06, belanger2016structured}:
\begin{align}
E_{\Theta}: \Xspace \times \yspace \rightarrow \mathbb{R} 
\end{align}
is parameterized by $\Theta$ that uses a functional architecture to compute a scalar energy for an input/output pair. The energy function can be an arbitrary function of the entire input/output pair, such as a deep neural network.



Given an energy function, the inference step is to find the output with lowest energy:
\begin{align}\label{eq:inf}
\hat{\y} = \argmin_{\y\in\yspace(\x)}E_{\Theta}(\x, \y)
\end{align}
However, solving Eq.~\eqref{eq:inf} requires combinatorial algorithms because $\yspace$ is a discrete structured space. This becomes intractable when $E_{\Theta}$ does not decompose into a sum over small ``parts'' of $\y$.   



Several special cases for $E_\Theta$:
\vspace{0.6cm}
\begin{itemize}
    \item Local classifiers $E_\Theta(\x, \y) = -\sum_i \log P_\Theta(y_i \mid F_i(\x))$:\\ \quad -- Decoding independently over all positions.
    \vspace{0.6cm}
    \item Linear chain CRFs~\citep{Lafferty:2001:CRF}  $E_{\Theta}(\x, \y) = -\left(\sum_{t} \sum_{i=1}^L y_{t,i} \left(U_i^\top f(\x,t)\right) + \sum_{t}\y_{t-1}^\top W \y_{t}\right)$ : \\ \quad --  Viterbi algorithm \small{[Viterbi, 1967]} 
    \vspace{0.6cm}
    \item Complex energy~\citep{belanger2016structured} : \\
    \quad -- \citet{belanger2016structured} relax this problem by allowing the discrete vector $\y$ to be continuous. Gradient descent for inference is used.
    \vspace{0.6cm}
\end{itemize}


\paragraph{Gradient Descent for Inference.}
\label{sec:gd}
\citet{belanger2016structured} uses gradient descent for inference. To use gradient descent (GD) for structured inference, researchers typically relax the output space from a discrete, combinatorial space to a continuous one and then use gradient descent to solve the following optimization problem: 
\begin{align}
%\y \approx
\argmin_{\y\in\relyspace(\x)}E_\Theta(\x, \y) \nonumber  %\label{eq:infnetFirst}
\end{align}
where $\relyspace$ is the relaxed continuous output space. For sequence labeling, $\relyspace(\x)$ consists of length-$|\x|$ sequences of probability distributions over output labels. 
To obtain a discrete labeling for evaluation, the most probable label at each position is returned. 

We actually perform gradient descent in an even more relaxed output space $\relyspacer(\x)$ which consists of length-$|\x|$ sequences of vectors, where each vector $\yv_t\in\mathbb{R}^L$,  $L$ is the label set size.
When computing the energy, we use a softmax transformation on each $\yv_t$, solving the following optimization problem with gradient descent:
\begin{align}
%\GD(\x)  = 
\argmin_{{\y}\in\relyspacer(\x)}E_\Theta(\x, \softmax({\y})) 
\label{eq:gdinf}
\end{align}
where the softmax operation above is applied independently to each vector $\yv_t$ in the output structure $\y$. 




==> ProposedMethods.tex <==
\section{Proposed Works}
\label{sec:proposed}
Previously, we replace the use of gradient descent with a neural network trained to approximate structured argmax inference. This inference network outputs continuous values that we treat as the output structure. According to the experiment results on several NLP tasks, including multi-label classification, part-of-speech tagging, named entity recognition, inference networks achieve a better speed/accuracy/search error trade-off than gradient descent, while also being faster than exact inference at similar accuracy levels. 

In this section, we propose several future directions.

\subsection{Exploring Energy Terms}
In section~\ref{sec:SPENTraining} and ~\ref{sec:jointobjective}, we use the linear-chain CRF energy and Tag Language model for sequence labeling task. In Section~\ref{sec:ENGINE}, we only use the pretrained autoregressive model as the energy function. It is worth to explore some other energy terms to capture complex label dependency. These terms can be used for sequence labeling or text generation tasks.

\paragraph{Skip Chain Energy}
We also consider an energy inspired by ``skip-chain'' conditional random fields~\citep{sutton04skip}. In addition to consecutive labels, this energy also considers pairs of labels appearing in a given window size $M+1$:
\begin{align}
%\label{eqn:energy-sequence-labeling1}
E_{W}( \y) = \sum_{t=1}^T \sum_{i=1}^M \y_{t-i}^\top W_i \y_{t}  \nonumber
\end{align}
where each $W_i\in\mathbb{R}^{L \times L}$ and the max window size $M$ is a hyperparameter. While linear chain energies allow efficient exact inference, using skip-chain energies causes exact inference to require time exponential in the size of $M$.


\paragraph{High Order Score function}
We also consider $M$th-order energy terms. We use the function $F$ to score the $M+1$ consecutive labels $\y_{t-M}, \dots, \y_{t}$, then sum over positions:  
\begin{align}
E_{W}( \y) = \sum_{t=M}^T F(\y_{t-M},\dots,\y_t) 
\label{eqn:high-order}
\end{align}
Convolutional neural networks (CNN)  are frequently used in NLP to extract features based on words or characters~\citep{2011:NLP-sm,kim-2014-convolutional}. We apply CNN filers over the sequence of $M+1$ consecutive labels. 
The $F$ function is computed as follows:
\begin{align}
&F(\y_{t-M},\dots,\y_t) = \sum_n f_{n}(\y_{t-M},\dots,\y_t) \nonumber \\
&f_{n}(\y_{t-M},\dots,\y_t) = g(W_n [\y_{t-M};
...;\y_{t} ] +\mathbf{b}_n)  \nonumber
\end{align}
\noindent where $g$ is a ReLU nonlinearity and the vector $W_n \in\mathbb{R}^{L(M+1)}$ and scalar $b_n \in\mathbb{R}$ are the parameters for filter $n$. 
The filter size of all filters is the same as the window size, namely, $M+1$. The $F$ function sums over all CNN filters. When viewing this high-order energy as a CNN, we can think of the summation as corresponding to sum pooling over time of the feature map outputs.


\paragraph{Reverse Score} The neural generation system~\citep{LiGBGD15} could rerank the outputs from the n-best list by linearly combining the forward score $p(\y \mid \x)$ and the ``reverse score'' $p(\x \mid \y)$, where the latter comes from a separately-trained seq2seq model. 
\begin{align}
    E_{\Theta}(\x, \y) = \sum_{t=1}^{|\x|} \log p_{\Theta}(x_t \mid \x_{0:t-1}, \y)
\end{align}
As we have discussed in the above subsection, a reverse generalized energy could be used during the training.

\paragraph{Language Coherence Terms} The way to improve the language coherence, we could use an additional energy term, the log-likelihood of y under the pretrained language models. The standard LSTM language model or the masked language model(e.g., BERT~\citep{devlin2018bert}, RoBERTa~\citep{roberta}).
The pretrained language models are the vital resources to exploit large monolingual corpora for NMT in our framework.

Another approach for the repetition is modeling coverage of the source sentence~\citep{tu-etal-2016-modeling,mi-etal-2016-coverage}. And \citet{holtzman-etal-2018-learning} designed an energy term specifically targeting the prevention of repetition in the output.

\paragraph{Relating Attention to Alignment}
Since the learned attention function may diverge from alignment patterns between languages, several researchers have experimented with adding inductive biases to the attention function~\citep{cohn-etal-2016-incorporating,feng-etal-2016-improving}. This is often motivated by known characteristics about the alignment between the source and target language, particularly those related to monotonicity, distortion, and fertility. It is worth to try similar terms with ~\citep{cohn-etal-2016-incorporating,feng-etal-2016-improving}.

\paragraph{Local Cross Entropy Term} The standard log-likelihood scoring function that is used by nearly all NMT systems. However, it is still not explored how to incorporate the standard cross entropy term with the other proposed energy terms. According to sequence labeling experiments results in Section~\ref{sec:SPENTraining}, the local cross entropy loss could contribute the performance of the inference networks. However, the weight for the term need to carefully tuned in the Section~\ref{sec:benchmark}, we use the weight annealing scheme). 

However, the local cross entropy term has some limitations: it does not assign partial credit to the hypotheses if the word order of hypotheses is different from the reference and it could penalize semantically correct hypotheses if they differ lexically from the reference. 

\paragraph{BLEU}
Recently, there are several work that directly optimize the evaluation metrics such as BLEU to improve the translation systems. The only issue is that we need to consider how to backpropagating through the term. With the similar approximate BLEU from ~\citet{tromble-etal-2008-lattice}, we could directly optimized the BLEU score for translation task or other generation tasks. 


\paragraph{Beyond BLEU} ~\citet{wieting-etal-2019-beyond} proposes a new metric based on semantic similarity in order to get partial credit and reduces the penalties on semantically correct hypotheses. This term could potentially lead the inference networks search better hypotheses with semantically similar hypotheses. The embedding model to evaluate similarity allows the range of possible scores to be continuous. The inference networks could get the gradient directly from the term.
\begin{align}
    SIM(r, h) = \mathrm{cos}(g(r), g(h))
\end{align}
\noindent where $r$ is the reference and $h$ are the generate hypothesis. $g$ is the encoder for a token sequence. 
Furthermore, one variation of the metric could be based on the semantic similarity between the source sentence and the hypotheses. This term potentially fine-tuning the hypotheses that have different semantic meaning from source sentence.  



\subsection{Other Training Methods for Energy-based Models}

\paragraph{Noise Contrastive Estimation}

In Section~\ref{sec:SPENTraining}, we use margin-based training metic(SSVM) for the energy function training. The objective for the energy function is:
\begin{align}
\Theta \gets & \argmin_{\Theta}\big[\cost(\canet(\x), \y_i) \!-\! E_{\Theta}(\x_i,\canet(\x)) + E_{\Theta}(\x_i, \y_i)\big]_{+} \nonumber
\end{align}

or in Section~\ref{sec:jointobjective} if jointly training two inference networks,

\begin{align}
\small
\begin{split}
\Theta \gets \argmin_{\Theta} \big[\cost(\canet(\x), \y_i) \!-\! E_{\Theta}(\x_i,\canet(\x)) + E_{\Theta}(\x_i, \y_i)\big]_{+}  + \lambda \big[- E_{\Theta}(\x_i,\infnet(\x_i)) + E_{\Theta}(\x_i, \y_i)\big]_{+} \nonumber
\end{split}
\end{align}

There is also other approach for energy training, noise-contrastive estimation~\citep{pmlr-v9-gutmann10a,ouSLT2018,ouICASSP2018,bakhtin2020energybased}  (NCE). 
NCE is proposed for learning unnormalized statistical models. It use logistic regression to discriminate between the data samples drawn from the data distribution and noise samples drawn from a noise distribution. If we use inference network output $\infnet$ as the noise sample distribution $P_{\Psi}$.
\begin{align}
    \max_{\Theta} \mathbb{E}_{(\x_i,\y_i) \in P_{\mathcal{D}}} \log \frac{1}{1 + \exp(E_{\Theta}(\x_i, \y_i))} + \mathbb{E}_{(\x_i,\y) \in P_{\infnet}} \log \frac{1}{1 + \exp(-E_{\Theta}(\x_i, \y))} \nonumber
\end{align}
\noindent where $P_{\mathcal{D}}$ is the data distribution and $P_{\infnet}$ is the output distributions from the inference network $\infnet$ (to improving sampling procedure, Langevin dynamics~\citep{WelTeh2011a} can be used).

The objective for inference networks is:
\begin{align}
\infnet(\x) \approx \argmin_{\y\in\relyspace(\x)}E_\Theta(\x, \y) \nonumber
\end{align}

We still can treat this optimization problem as minmax game and find a saddle point for the game. Following \citet{goodfellow2014generative} and Section~\ref{sec:SPENTraining}, we alternate between one mini-batch for optimizing $\Psi$ and one for optimizing $\Theta$.

\paragraph{Deep Value Network}

Deep value network~\citep{DVNGygliNA17} directly train a neural network $v(\x, \y, \theta)$ to accurately predict the desired performance metrics(e.g., IOU). It use a different objective that encourages the score to equal the task loss of the prediction. In the ~\citet{DVNGygliNA17}, the objective is to correctly predict the F1 score for any potential label configuration. The similar approximate BLEU score from~\citep{tromble-etal-2008-lattice} could be used for machine translation task.

The training goal is, 
\begin{align}
   v(\x, \y, \theta) \approx & v(\y, \y^*) = -l(\y, \y^*) \\ \nonumber
\end{align}
Where $l$ is the loss function $l(\y, \y^*)$ that compares an output $\y$ against a ground truth label $\y^*$. It could be the F1 or BLEU score.


The training objective is\footnote{~\citet{DVNGygliNA17} also demonstrate the other loss function can be used, e.g., L2}, 
\begin{align}
   L =& \sum_{(\x,\y,v^*) \in \mathcal{D}} -v^* \log v(\x,\y) -(1-v^*) \log(1-v(\x,\y))
\end{align}
Where $\y$ is the generated example given a training example $(\x, \y^*)$.  $v^*$ is oracle value for $y$ (it is the loss $-l(\y, \y^*)$). $\y$ could be generated with gradient based inference, random samples, or adversarial training in Section~\ref{sec:SPENTraining}. 

In order to infer a prediction for an input $\x$, we need to find the $\hat{y}$:
\begin{align}
  \hat{y} = \argmax_{\y} v(\x, \y, \theta) 
\end{align}

With the similar approximate BLEU from ~\citet{tromble-etal-2008-lattice}, we could directly optimized the BLEU score for translation task or other generation tasks.

\paragraph{Linear Corpus BLEU} Let $r$ be reference length, $c_0$ the candidate length, and $\{c_n | 1 \leq n \leq 4 \}$ the number of n-gram matches. Then the corpus BLUE score $B(r,c_0, c_n)$ can be defined as follows:
\begin{align}
\log B = & \min(0, 1-\frac{r}{c_0}) + 0.25*\sum_{n=1}^{4} \log\frac{c_n}{c_0 - \delta_n} \\ \nonumber
  \approx & \min(0, 1-\frac{r}{c_0}) + 0.25*\sum_{n=1}^{4} \log\frac{c_n}{c_0}
\end{align}
Where $\delta_n$ is ignored. If $L$ is the average sentence length in the corpus, $\delta_n \approx (n-1) \frac{c_0}{L}$.

% \subsection{How To Get Better Inference Networks} 
% It is worth to try with more robust autoregressive models as the energy functions, e.g., the pretrained state-of-art machine translation model. It is worth exploring whether the performance of the inference network is improved with better autoregressive models. How is the gap between the inference network and the pretrained model? Is it possible that the inference networks have better performance than the pretrained models?

% Another potential direction is to post processing the output of the inference network in case that the inference network is not optimized well. For example, the extra refinement steps could be done for the CMLM inference networks.


\subsection{Handling Constraints in Inference (eg. tree)}
 To improve inference speed, ~\citet{tu-18} learn a neural net to produce the same output with low energy. This approach does not permit to include known structure. We could focus on enforcing constraints at inference-time. Previous
work for enforcing constraints have focused on constrained $A^*$ decoding~\citep{he-etal-2017-deep} or integer linear programming~\citep{punyakanok-etal-2008-importance}, post-processing~\citep{NIPS2015_5635}, building them into
the decoder transitions~\citep{dyer-etal-2016-recurrent}, search constraints~\citep{wiseman-rush-2016-sequence}, Lagrangian
relaxation~\citep{koo-etal-2010-dual,LeeWTC17}.

\citet{pan-etal-2020-learning} proposed to use a two-layer rectifier network to identify valid structures or substructures. 
To obtain a parse given the span scores, We need to extract the maximum scoring parse tree.

\begin{align}
    \treescore(B, S) = \sum_{i \leq j} B_{ij} s_{ij} \nonumber
\end{align}
Where the score $s_{ij} \in \mathcal{R}$ for a constituent spanning $x_i$ to $x_j$ is given. $B$ be the binary matrix representation of a tree($B_{ij}$ means there is a constituent spanning $x_i$ ans $x_j$)

During the inference, we try to find the tree $B$ with maximum $\treescore(B, S)$:
\begin{align}
    \argmax_B \treescore(B, S) = \sum_{i \leq j} B_{ij}s_{ij} \nonumber
\end{align}

Previously, it is done based on our single grammar rule using the CKY procedure~\citep{Kas}. Runtime complexity for CKY in terms of sentence length $n$ is $\mathcal{O}(n^3)$. We can use inference network which output a tree $B$ with max tree score. The tree $B$ can be the output of shift-reduce parser.

given the spanning score, we could train the inference network that could minic the process:
\begin{align}
    \argmax_{\Psi} \sum_{\langle x, S\rangle \in \mathcal{D}} \treescore(\infnet(x, S), S)
\end{align}
\noindent where $\mathcal{D}$ are the training data pairs including the sentences and spanning scores. $\infnet$ can be shift-reduce parser that do parallel decoding, and output a tree with maximum tree score at the same time.
% \begin{algorithm}
% \caption{CKY algoritm: Viterbi algorithm}
% \begin{algorithmic} 
% \REQUIRE SCORE: scores for each span
% \STATE Calculate a maximum score for each span,
% and record a backpointer
% \FOR {i = 1 to n}
%     \STATE chart[i, i] $\leftarrow$ SCORE[i,i]
% \ENDFOR
% \FOR {width = 2 to n}
%     \FOR {start = 0 to n - width}
%         \STATE end $\leftarrow$ start + width
%         \STATE mid = start to end-1
%         %\STATE chart[start, end] max = $\min_{\mathrm{mid}}$ chart[start, mid]+ chat[mid, end]
%         \STATE chart[start, end] = $\max_{\mathrm{mid}}$ chart[start, mid]+ chat[mid+1, end] + SCORE[start, end]
%     \ENDFOR
% \ENDFOR
% \RETURN chart[0, n]
% \end{algorithmic}
% \end{algorithm}


\subsection{Minimum Risk Decoding}
 ~\citep{kumar-byrne-2004-minimum,tromble-etal-2008-lattice} presents the results show that MBR decoding can be used to tune statistical MT performance for specific loss function. In the field of machine translation, the technique was originally developed for rescoring k-best lists of hypotheses generated by a statistical model.
\begin{align}
\hat{E} =& \argmin_{E' \in \xi_h} R(E') \nonumber \\ 
        = & \argmin_{E' \in \xi_h} \sum_{E \in \xi_e} L(E, E')P(E \mid F) \nonumber
\end{align}
where $R(E')$ denotes the Bayes risk candidate translation $E'$ under the loss function $L$. $\xi_h$ refers to the Hypothesis space from where the translations are chosen. $\xi_e$ refers to the Evidence space that is used for computing the Bayes risk. ~\citet{tromble-etal-2008-lattice}, showed that the Lattice MBR decoder yields moderate, consistent gains in translation performance over N-best MBR decoding on several language pairs. There are two potential reasons that MBR decoding could outperform N-best MBR: a larger hypothesis space or a better posterior distribution over translation hypotheses.

Enable efficient implementation of the decoder on such large search spaces is really difficult. Further exploration could be done in the above directions. For example, an inference network $\infnet$ which maps an input $F$ to a translation $E$ and 
is trained with the goal that:
\begin{align}
    \infnet(F) \approx \argmin_{E' \in \xi_h} \sum_{E \in \xi_e} L(E, E')P(E \mid F)
\end{align}
Then, given the probability model $P(E \mid F)$, we could train the inference network that could minic MBR decoding with the following objective:
\begin{align}
    \argmin_{\Psi} \sum_{F \in \mathcal{D}} \sum_{E \in \xi_e} L(E, \infnet(F))P(E \mid F)
\end{align}
 \noindent where $\mathcal{D}$ could be training data or test data without the reference. A good inference network can be first trained on the training data. And the inference network can be also fine-tuned on the test data with good starting point which is trained on the training data.  


\subsection{Timeline}

The Table~\ref{tab:timeline} shows a rough timeline when I plan to do the particular proposed work components.

\begin{table}[h!]
  \begin{center}
    \label{tab:table1}
    \begin{tabular}{l|c|}
      \textbf{Proposed work} & \textbf{Timeline}\\
      %$\alpha$ & $\beta$ & $\gamma$ \\
      \hline
       explore energy functions & March-Sep 2020 \\
       Energy model training & March - Sep 2020 \\
       constrained decoding  & March -Dec 2020  \\
       Minimum Risk Decoding & July - Dec 2020   \\ \hline
       \textbf{Dissertation} (expected)               & Dec 2020    \\        \hline
    \end{tabular}
    \caption{\label{tab:timeline} Timeline for the proposed work}
  \end{center} 
\end{table}

==> approach.tex <==

\section{Proposed work}

\subsection{Exploring Energy Functions for Generation.}
NMT,
1. The best model autoregressive models  better inference network
2. adding LM terms
3. repeatation energy, coverage

4. CMLM refinements for the inference network
5. adding CE?


\subsection{Minum risk decoding}
tagging, parsing, posterior decoding


\subsection{constrained decoding (eg.tree)}

\subsection{Marginal inference}

\subsection{Language Model for Generation}


\paragraph{Ensemblling Elmo, Bert and GPT.}
%Background of Knowledge Distillation
\citet{hinton2015distilling} proposed a knowledge distillation method. it has two terms in the loss: 

\begin{align}
\loss = \ce(y, P_{\Theta}) + \lambda \lkd(P_{\Psi}, P_{\Theta}) \nonumber 
\end{align}
Here $y$ is the ground-truth label, $P_{\Theta}$ is output probability of the student network and $P_{\Psi}$ is output probability of the teacher network
One is the cross-entropy between the output a student network and labels, the other is cross-entropy between outputs of a student network and the softened output of the teacher network.

The second term could be also written as following:
\begin{align}
\lkd(P_{\Psi}, P_{\Theta}) = -\sum P_{\Psi} \log \frac{P_{\Theta}}{P_{\Psi}} \nonumber
\end{align}
\paragraph{language model for Generation.}
especially for low-resource MT


comparing with conditional GAN?


\subsection{COn}






==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\Softmax}{\mathrm{Softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> misc.tex <==
\subsection{Probabilistic versus Non-Probabilistic}

\textbf{Probabilistic objective}
\textbf{directly maximizing the likelihood of the data} 

\textbf{hinge loss (Reranking, Contrastive Estimation~\citet{smith-eisner-2005-contrastive})} : “soft” version of the hinge loss with an infinite margin~\citep{lecun-06} do not
attempt to model class membership probability
~\citet{journals/jmlr/CollobertWBKKK11}: ranking loss to learn word embedding:
~\citet{smith-eisner-2005-contrastive} a contrastive criterion which estimates the likelihood of the data conditioned t


\textbf{``inject domain
knowledge``: not only the observed positive example, but also a set of similar but deprecated negative
examples}
\begin{itemize}
    \item computation cost
    \item inductive bias
\end{itemize}

(Smith, 2011), such as cost-augmented
decoding, can be easily applied or adapted to the neural-network framework: One should keep in mind that the resulting objectives are no longer convex, and so lack the formal guarantees and bounds associated with convex optimization problems. Similarly, the theory, learning bounds
and guarantees associated with the algorithms do not automatically transfer to the neural versions.

\textbf{It is therefore desirable to define alternative training criteria. We propose here to use a pairwise
ranking approach (Cohen et al., 1998). We seek a network that computes a higher score when
given a legal phrase than when given an incorrect phrase. Because the ranking literature often deals
with information retrieval applications, many authors define complex ranking criteria that give more
weight to the ordering of the best ranking instances (see Burges et al., 2007; Clemenc¸on and Vayatis, ´
2007). However, in our case, we do not want to emphasize the most common phrase over the rare
but legal phrases. Therefore we use a simple pairwise criterion.}


\textbf{This is because the search is intractable and/or exact maximization has some undesirable quality (e.g., it’s in fact an
alternative viable prediction). In this case, maximization is replaced by sampling}




\paragraph{Discussion why we consider deep structure.}



energy-based model with latent variables and auto-encoder was discovered by 

Contrastive Divergence~\citet{Contrastive}

a much more general method than score matching
since it is applicable to intractable latent variable models. It can also handle binary/discrete
variables 


training other probabilistic discriminative sequence labeling: HMM and CRF

This idea is the basis of the contrastive divergence algorithm proposed by
Hinton [Hinton, 2002]. Contrastive divergence learning can be seen as an approximation of NLL learning with two shortcuts using a Markov chain Monte Carlo method.  The basic principle is to use an MCMC method for computing
the derivative of the logarithm of the normalization factor Z



Probabilistic Density Models 

language model 

score matching estimator~\citet{hyvarinen05a} unnormalized density models over continuous-valued data. Score matching is thus preferable if a consistent estimator is
wanted.  ~\citet{vaeScoreMatch} connections from VAE score machting

Markov Random Fields and Conditional Random Fields
VAE~\citep{vaeScoreMatch}


~\citep{ZhaoML16} framework as using an auto-encoder architecture. propose learning a separate network to generate samples\\

auto-encoders VAE and energy-based model ~\citet{xiao2021vaebm}
% probability model

better than LSTM-based language model

~\citet{pmlr-v2-ranzato07a}  Unsupervised Learning where the energy should be increased or implicitly via global constraints such as sparsity


\textbf{amortized generation is prone to mode collapse, especially when
training the sampling network without an entropy term which is often approximated or ignored. Approximate inference methods can also be used during training, though the energy function may incorrectly assign low energy to some modes if the approximate inference method cannot find them.} \\ 

Linear Structured Models: CRF, SVMM, and MMMN

Out-of-distribution


catastrophic collapse: nonprobabilistic 

structured application


\textbf{in applications where calibration is important (i.e. you want an estimate of the true posterior probability, this is a natural fit. SVMs do not directly model the probability, though one can actually obtain this in practice via calibratio}

~\citep{FinnCAL16}: the interpretation of GANs as an algorithm for training energy-based models, and relate this interpretation to other recent work that seeks to connect GANs
and EBMs.

\paragraph{Sequence Modeling.} 
Energy Networks have been used for sequence modeling.


\paragraph{Conditional Modeling.}

\paragraph{Normalize}
the energy function does not need to be trained as a probabilistic
model, and each factor does not need to correspond to a locally-normalized distribution.

\paragraph{Unnormalize}

